Improving Inductive Link Prediction Using Hyper-Relational Facts

For many years, link prediction on knowledge graphs (KGs) has been a purely transductive task, not allowing for reasoning on unseen entities. Recently, increasing efforts are put into exploring semi- and fully inductive scenarios, enabling inference over unseen and emerging entities. Still, all these approaches only consider triple-based \glspl{kg}, whereas their richer counterparts, hyper-relational KGs (e.g., Wikidata), have not yet been properly studied. In this work, we classify different inductive settings and study the benefits of employing hyper-relational KGs on a wide range of semi- and fully inductive link prediction tasks powered by recent advancements in graph neural networks. Our experiments on a novel set of benchmarks show that qualifiers over typed edges can lead to performance improvements of 6% of absolute gains (for the Hits@10 metric) compared to triple-only baselines. Our code is available at \url{https://github.com/mali-git/hyper_relational_ilp}.

==> generated/100_v1_qualifier_relations_impact.tex <==
%\begin{tabular}{llr}
%\toprule
Wikidata ID & relation name &   $\Delta$MR \\
\midrule
         P2868 &        subject has role &   0.12 \\
          P463 &               member of &  -0.04 \\
         P1552 &             has quality &  -0.34 \\
        %  P2936 &           language used &  -0.38 \\
        %   P929 &             color space &  -0.61 \\
          \midrule
        %   P20 &          place of death & -18.33 \\
        %  P2293 &     genetic association & -23.42 \\
         P2241 &  reason for deprecation & -26.44 \\
           P47 &      shares border with & -28.91 \\
          P750 &          distributed by & -29.12 \\
%\bottomrule
%\end{tabular}

==> generated/66_v2_qualifier_relations_impact.tex <==
%\begin{tabular}{llr}
%\toprule
%Wikidata ID & relation name & $\Delta$MR \\
%\midrule
          P805 &  statement is subject of &  13.11 \\
         P1012 &                including &   5.95 \\
          P812 &           academic major &   5.07 \\
        %  P2541 &           operating area &   2.57 \\
        %  P1399 &             convicted of &   2.41 \\
         \midrule
        %  P1622 &             driving side &  -6.44 \\
        %  P1546 &                    motto &  -8.09 \\
           P17 &                  country & -19.96 \\
         P1310 &    statement disputed by & -20.92 \\
         P1686 &                 for work & -56.87 \\
%\bottomrule
%\end{tabular}

==> macros.tex <==


\newcommand{\rel}{\mathcal{R}\xspace}
\newcommand{\en}{\mathcal{E}\xspace}
\newcommand{\eh}{\mathcal{E}_H\xspace}
\newcommand{\et}{\mathcal{E}_T\xspace}
\newcommand{\equ}{\mathcal{E}_Q\xspace}
\newcommand{\es}{\mathcal{E}_{\bullet}\xspace}
\newcommand{\eu}{\mathcal{E}_{\circ}\xspace}

\newcommand{\strain}{\mathcal{S}_{train}\xspace}
\newcommand{\seval}{\mathcal{S}_{eval}\xspace}
\newcommand{\sinf}{\mathcal{S}_{\mathit{inf}}\xspace}

\newcommand{\pset}{\mathfrak{P}\xspace}


